Counter-terrorism in cyber-physical spaces: Best practices and technologies from the state of the art

Context: The demand for protection and security of physical spaces and urban areas increased with the escalation of terroristic attacks in recent years. We envision with the proposed cyber-physical systems and spaces, a city that would indeed become a smarter urbanistic object, proactively providing alerts and being protective against any threat. Objectives: This survey intend to provide a systematic multivocal literature survey comprised of an updated, comprehensive and timely overview of state of the art in counter-terrorism cyber-physical systems, hence aimed at the protection of cyber-physical spaces. Hence, provide guidelines to law enforcement agencies and practitioners providing a description of technologies and best practices for the protection of public spaces. Methods: We analyzed 112 papers collected from different online sources, both from the academic field and from websites and blogs ranging from 2004 till mid-2022. Results: a) There is no one single bullet-proof solution available for the protection of public spaces. b) From our analysis we found three major active fields for the protection of public spaces: Information Technologies, Architectural approaches, Organizational field. c) While the academic suggest best practices and methodologies for the protection of urban areas, the market did not provide any type of implementation of such suggested approaches, which shows a lack of fertilization between academia and industry. Conclusion: The overall analysis has led us to state that there is no one single solution available, conversely, multiple methods and techniques can be put in place to guarantee safety and security in public spaces. The techniques range from architectural design to rethink the design of public spaces keeping security into account in continuity, to emerging technologies such as AI and predictive surveillance.

==> sections/0_abstract.tex <==
The demand for protection and security of physical spaces and urban areas increased with the escalation of terroristic attacks in recent years and to mitigate crimes like pickpocketing, harassment, public violence, or mob control. Our systematic literature review aims to provide an overview of cyber-physical systems technologies available to protect public spaces. We analyzed 112 papers collected from different online sources, both from the academic field and from websites and blogs ranging from 2004 until mid-2022. The overall analysis has led us to state that there is no one single solution available, conversely, multiple methods and techniques can be put in place to guarantee safety and security in public spaces. The techniques range from architectural design to rethinking the design of public spaces keeping security into account in continuity, to emerging technologies such as AI and predictive surveillance. Moreover, whenever new technologies appear to be expensive in cost and questionable regarding privacy or when it could be difficult to rethink and re-project public spaces, building an action plan to mitigate, prevent, and manage crime events would be a viable solution.
